Optimization over Nonnegative and Convex Polynomials With and Without Semidefinite Programming

The problem of optimizing over the cone of nonnegative polynomials is a fundamental problem in computational mathematics, with applications to polynomial optimization, control, machine learning, game theory, and combinatorics, among others. A number of breakthrough papers in the early 2000s showed that this problem, long thought to be out of reach, could be tackled by using sum of squares programming. This technique however has proved to be expensive for large-scale problems, as it involves solving large semidefinite programs (SDPs). In the first part of this thesis, we present two methods for approximately solving large-scale sum of squares programs that dispense altogether with semidefinite programming and only involve solving a sequence of linear or second order cone programs generated in an adaptive fashion. We then focus on the problem of finding tight lower bounds on polynomial optimization problems (POPs), a fundamental task in this area that is most commonly handled through the use of SDP-based sum of squares hierarchies (e.g., due to Lasserre and Parrilo). In contrast to previous approaches, we provide the first theoretical framework for constructing converging hierarchies of lower bounds on POPs whose computation simply requires the ability to multiply certain fixed polynomials together and to check nonnegativity of the coefficients of their product. In the second part of this thesis, we focus on the theory and applications of the problem of optimizing over convex polynomials, a subcase of the problem of optimizing over nonnegative polynomials. (See manuscript for the rest of the abstract.)

==> ch-intro/intro_contributions.tex <==
This document serves as a template to demonstrate how to use the \texttt{puthesis} documentclass for a Princeton University Ph.D.\ Disseration. Some of the requirements for a master's thesis or an undergraduate thesis are different, especially the text on the title page, so you will need to make some modifications to use this template for those purposes. 

This template is setup to easily make a few different versions of your dissertation. The version you will print and have bound should generally be single spaced (and single-sided), and not contain any hyperlinks. The electronic version that you submit to your readers to review and to be published by ProQuest will be double spaced, and will contain PDF features such as bookmarks for each section and internal links to citations, footnotes, and other internal references.  

During the writing process, you may want to disable some of the frontmatter (list of tables, list of figures, acknowledgements, and maybe even the table of contents. I have not tested this template with equations or a list of symbols, but those are available.
